What Players do with the Ball: A Physically Constrained Interaction Modeling

Tracking the ball is critical for video-based analysis of team sports. However, it is difficult, especially in low-resolution images, due to the small size of the ball, its speed that creates motion blur, and its often being occluded by players. In this paper, we propose a generic and principled approach to modeling the interaction between the ball and the players while also imposing appropriate physical constraints on the ball's trajectory. We show that our approach, formulated in terms of a Mixed Integer Program, is more robust and more accurate than several state-of-the-art approaches on real-life volleyball, basketball, and soccer sequences.

==> Figures/EA_table.tex <==
\begin{table}[!h]
    \begin{tabular}{|p{1.3cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{1cm}|p{0.9cm}|}
\hline
Dataset:    &  \multicolumn{2}{c|}{\volley{}} & \multicolumn{3}{c|}{\basket{}} & \soccer{} \\ 
\hline
Approach:   &    1   & 2 & 1 & 2 & APIDIS & ISSIA \\
\hline
\our{}      & 0.77 & 0.80 & 0.66 & 0.63 & 0.64 & 0.49 \\
\hline
\ournp{}    & 0.77 & 0.68 & 0.59 & 0.40 & 0.57 & 0.48 \\
\hline
\ourns{}    & 0.73 & 0.63 & 0.50 & 0.33 & 0.49 & 0.49 \\
\hline
\inter{}    & 0.68 & 0.65 & 0.55 & 0.33 & 0.49 & 0.45 \\
\hline
\ksp{}      & 0.67 & 0.58 & 0.48 & 0.30 & 0.47 & 0.39 \\
\hline
{\bf MaxDe- tection}   & 0.54 & 0.53 & 0.39 & 0.25 & 0.42 & 0.25 \\
\hline
\ransac{}   & 0.65 & 0.56 & 0.42 & 0.27 & 0.46 & 0.25 \\
\hline
\growth{}   & ???  & ???  & --- & --- & --- & --- \\
\hline
\end{tabular}
\caption{Event accuracy for different methods and datasets.}
\label{tab:EAtable}
\end{table}

\comment{
\begin{table}
\begin{tabular}{|l|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|}
\hline
Dataset & \our{} & \ournp{} & \ourns{} & \inter{} & \ksp{} & \maxdet{}  & \ransac{} \\
\hline
\volley{1} & 0.77 & 0.77 & 0.73 & 0.68 & 0.67 & 0.65 & 0.54 \\
\hline
\volley{2} & 0.80 & 0.68 & 0.63 & 0.65 & 0.58 & 0.56 & 0.53 \\
\hline
\basket{1} & 0.66 & 0.59 & 0.50 & 0.55 & 0.48 & 0.42 & 0.39 \\
\hline
\basket{2} & 0.63 & 0.40 & 0.33 & 0.33 & 0.30 & 0.27 & 0.25 \\
\hline
\basket{APIDIS} & 0.64 & 0.57 & 0.49 & 0.49 & 0.47 & 0.46 & 0.42 \\
\hline
\soccer{ISSIA} & 0.49 & 0.48 & 0.49 & 0.45 & 0.39 & 0.25 & 0.25 \\
\hline
\end{tabular}
\caption{Event accuracy for different methods and datasets. \amrmk{As it is quite likely that this table will not go into the paper, I did not format the header properly. Will do so as needed.}}
\label{tab:EAtable}
\end{table}
}


==> Figures/TA_table.tex <==
\comment{
Volley1
\begin{tabular}{|l|c|c|c|c|}
    \hline
    Method              &       $TA(30cm)$   &   $TA(100cm)$   &   $EA(5 fr.)$   \\ 
    \hline
    OUR                 &       0.790        &    0.933        &                 \\
    \hline
    \ournp{}            &       0.792        &    0.908        &                 \\
    \hline
    \ourns{}            &       0.650        &    0.846        &                 \\
    \hline
    MIP                 &       0.678        &    0.858        &                 \\
    \hline
    KSP                 &       0.577        &    0.754        &                 \\
    \hline
    MaxDetection        &       0.421        &    0.515        &                 \\
    \hline
    FoS                 &       -----        &    -----        &                 \\
    \hline
    RANSAC              &       0.695        &    0.840        &                 \\
    \hline
    CompTrack           &       0.029        &    0.041        &                 \\
    \hline
\end{tabular}
}

\begin{table}[t]
\begin{tabular}{|l|c|c|c|c|}
    \hline
    Method              &       $TA(30cm)$   &   $TA(100cm)$   &   $EA(5 fr.)$   \\ 
    \hline
    OUR                 & \textbf{0.684}     &  \textbf{0.861} &                 \\
    \hline
    \ournp{}            &       0.593        &    0.779        &                 \\
    \hline
    \ourns{}            &       0.451        &    0.642        &                 \\
    \hline
    MIP                 &       0.608        &    0.678        &                 \\
    \hline
    KSP                 &       0.585        &    0.643        &                 \\
    \hline
    MaxDetection        &       0.293        &    0.479        &                 \\
    \hline
    FoS                 &       -----        &    -----        &                 \\
    \hline
    RANSAC              &       0.591        &    0.777        &                 \\
    \hline
    CompTrack           &       0.024        &    0.032        &                 \\
    \hline
\end{tabular}
\caption{Tracking and event accuracy on Volley2 dataset}
\label{tab:TAvolley2}
\end{table}

\comment{
FIBAW1
\begin{tabular}{|l|c|c|c|c|}
    \hline
    Method              &       $TA(30cm)$   &   $TA(100cm)$   &   $EA(5 fr.)$   \\ 
    \hline
    OUR                 &       0.707        &    0.802        &                 \\
    \hline
    \ournp{}            &       0.620        &    0.742        &                 \\
    \hline
    \ourns{}            &       0.548        &    0.661        &                 \\
    \hline
    MIP                 &       0.691        &    0.735        &                 \\
    \hline
    KSP                 &       0.621        &    0.665        &                 \\
    \hline
    MaxDetection        &       0.505        &    0.596        &                 \\
    \hline
    FoS                 &       0.684        &    0.828        &                 \\
    \hline
    RANSAC              &       0.555        &    0.633        &                 \\
    \hline
    CompTrack           &       0.000        &    0.006        &                 \\
    \hline
\end{tabular}
}


==> Figures/_w <==
% !TEX root = ../top.tex
\comment{
\begin{figure*}[t]
\begin{center}
\hspace{-1pt}
\begin{tabular}{ccc}
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.34\textwidth]{Figures/TA_Volley1.pdf} &
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.34\textwidth]{Figures/TA_Volley2.pdf} &
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.34\textwidth]{Figures/TA_Basket1.pdf}\\ 
	
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.34\textwidth]{Figures/TA_Basket2.pdf} &
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.34\textwidth]{Figures/TA_Apidis.pdf} &
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.34\textwidth]{Figures/TA_Issia.pdf}
   \\
\end{tabular}
\end{center}
\vspace{-3mm}
\caption{Ball Tracking Accuracy}
\label{fig:TAFigure}
\end{figure*}
}
% Space - optimized version
\begin{figure*}
\begin{center}
\hspace{-1pt}
\begin{tabular}{cccc}
   \hspace{-0.2cm} (a) &
   \hspace{-0.2cm} (b) &
   \hspace{-0.2cm} (c) &
   \hspace{-0.2cm} (d) \\
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.24\textwidth]{Figures/TA_Volley1.pdf} &
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.24\textwidth]{Figures/TA_Volley2.pdf} &
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.24\textwidth]{Figures/TA_Basket1.pdf} &	
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.24\textwidth]{Figures/TA_Basket2.pdf} \\ 


   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.24\textwidth]{Figures/TA_Apidis.pdf} &
   \hspace{-0.4cm}\includegraphics[trim={1.8cm 6.5cm 2.3cm 6.5cm},clip,width=0.24\textwidth]{Figures/TA_Issia.pdf} & \multicolumn{2}{c}{\includegraphics[trim={0 0 0 3cm},clip,width=0.48\textwidth]{Figures/event_accuracy_bar_2.pdf}} & 
   \vspace{-5mm}
   \\
   \vspace{-5mm}
   \hspace{-0.2cm} (e) &
   \hspace{-0.2cm} (f) &
   \hspace{-0.24\textwidth} \multicolumn{2}{c}{(g)} & \\
\end{tabular}
\end{center}
\vspace{-6mm}
\caption{Ball Tracking Accuracy}
\label{fig:TAFigure}
\end{figure*}



==> Figures/graphLayout.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.7\columnwidth]{Figures/graph_layout.png}
\caption{Example of graph nodes in three time frames. Bold edges correspond to
the transitions when the state of the ball changes.}
\label{fig:networkFlow}
\end{center}
\end{figure}

